Temporal Shift GAN for Large Scale Video Generation

Video generation models have become increasingly popular in the last few years, however the standard 2D architectures used today lack natural spatio-temporal modelling capabilities. In this paper, we present a network architecture for video generation that models spatio-temporal consistency without resorting to costly 3D architectures. The architecture facilitates information exchange between neighboring time points, which improves the temporal consistency of both the high level structure as well as the low-level details of the generated frames. The approach achieves state-of-the-art quantitative performance, as measured by the inception score on the UCF-101 dataset as well as better qualitative results. We also introduce a new quantitative measure (S3) that uses downstream tasks for evaluation. Moreover, we present a new multi-label dataset MaisToy, which enables us to evaluate the generalization of the model.

==> fig_memorization.tex <==
\iffalse
\begin{figure}[h]
\centering
\begin{subfigure}{.95\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{images/intra_figure.jpg}
  \caption{\methodshort.}
  \label{fig:tmm-intra1}
\end{subfigure}%
\vfill
\begin{subfigure}{.95\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{images/figure_intra_128.jpg}
  \caption{TSB.}
  \label{fig:tmm-intra2}
\end{subfigure}
%\vspace{-.8em}
\caption{Example of intra-class interpolation on UCF-101. The vertical axis represents time, the horizontal axis represents different modes of the class. We sample two latent codes which are represented by the leftmost and right most samples and linearly interpolate between them to generate intermediate latent code samples.}
\vspace{-.8em}
\label{fig:intra}
\end{figure}
\vspace{-.3em}
\fi

\begin{figure*}[h]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.86\linewidth]{images/figure_weiz_tsb.jpg}
\end{center}
   \caption{Generated samples on Weizmann dataset with our TSB model.}
   \vspace{-1em}
\label{fig:weiz_gen}
\end{figure*}
   \vspace{-18em}


\begin{figure}[h]
\centering
\begin{subfigure}{.95\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{images/inter_figure.jpg}
  \caption{\methodshort.}
  \label{fig:tmm-inter1}
\end{subfigure}%
\vfill
\begin{subfigure}{.95\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{images/inter_128_figure.jpg}
  \caption{TSB.}
  \label{fig:tmm-inter2}
\end{subfigure}

\caption{Interpolation Performance showing smooth transitions between classes on UCF-101. Each column is a sequence.(a) The top figure is interpolating between classes writing on board (left) and pole vault (right), while the bottom one is interpolating volleyball spiking (left) and frisbee catch (right). (b) The top figure is interpolating between classes basketball (left) and frisbee catch (right), while the bottom one is interpolating between golf swing (left) and diving (right).}
\vspace{-.8em}
\label{fig:inter}
\end{figure}
\vspace{-2mm}
\section{Conclusion}
\vspace{-2mm}
We presented a TSB architecture for video generation that enforces temporal consistency into a 2D video generator network. We show that TSB design improves the quality of generated videos in comparison to the BigGAN baseline. To validate effectiveness of our method, we conduct experiments on four different datasets including our new dataset MaisToy. Our new dataset enables us to analyze the generalization power of model and also understand which semantics are easier for model to learn.
As a supplement to the well established IS score, we proposed the generalization based S3 score, which is intended to be sensitive to intra-class variation. 
Based on this metric our method also achieves the best performance. These quantitative results are further supported by our qualitative.
\vspace{-1mm}

\section{Acknowledgements}
\vspace{-2mm}
We acknowledge funding by the German Research Foundation (DFG) via the
grant BR 3815/10-1 and the gift of a compute server by Facebook.


\begin{figure}[h!]
\centering
\begin{subfigure}{0.95\textwidth}
  \centering
  \includegraphics[width=0.95\linewidth]{images/crawl_swim_n.jpg}
  \caption{Front Crawl.}
  \label{fig:knn1}
\end{subfigure}%
\vfill
\begin{subfigure}{0.95\textwidth}
  \centering
  \includegraphics[width=0.95\linewidth]{images/snowboard_n.jpg}
  \caption{Skiing.}
  \label{fig:knn2}
\end{subfigure}
\vspace{-.4em}
\caption{ Examples of retrieval of top-3 nearest neighbors (black) of TSB generated samples (red). We can see that although the generated samples look similar to their respective 3-NNs, they are still quite visually distinct. This implies the model isn't just memorizing the real data.}
\label{fig:knn}
\end{figure}

\iffalse
\section{Acknowledgements}
\vspace{-2mm}
We acknowledge funding by the German Research Foundation (DFG) via the
grant BR 3815/10-1 and the gift of a compute server by Facebook.
\fi
